Partially Permuted Multi-Trellis Belief Propagation for Polar Codes

Belief propagation (BP) is an iterative decoding algorithm for polar codes which can be parallelized effectively to achieve higher throughput. However, because of the presence of error floor due to cycles and stopping sets in the factor graph, the performance of the BP decoder is far from the performance of state of the art cyclic redundancy check (CRC) aided successive cancellation list (CA-SCL) decoders. It has been shown that successive BP decoding on multiple permuted factor graphs, which is called the multi-trellis BP decoder, can improve the error performance. However, when permuting the entire factor graph, since the decoder dismisses the information from the previous permutation, the number of iterations required is significantly larger than that of the standard BP decoder. In this work, we propose a new variant of the multi-trellis BP decoder which permutes only a subgraph of the original factor graph. This enables the decoder to retain information of variable nodes in the subgraphs, which are not permuted, reducing the required number of iterations needed in-between the permutations. As a result, the proposed decoder can perform permutations more frequently, hence being more effective in mitigating the effect of cycles which cause oscillation errors. Experimental results show that for a polar code with block length 1024 and rate 0.5 the error performance gain of the proposed decoder at the frame error rate of 10^(-6) is 0.25 dB compared to multi-trellis decoder based on full permutations. This performance gain is achieved along with reduced latency in terms of the number of iterations.

==> algo.tex <==












\begin{algorithm}[h]
\SetAlgoLined
\DontPrintSemicolon
\SetKwInput{Input}{Input} 
\SetKwInput{Output}{Output} 
\Input
  {\begin{itemize}
  \setlength\itemsep{0em}
   \item[] {\makebox[2cm][l]{$\mathbf{L}_{1,j}$}      \% LLR channel output}
   \item[] {\makebox[2cm][l]{$\mathbb{A}$}  \% information set}
   \item[] {\makebox[2cm][l]{$P_{level}$} \% max. no. of stages to be permuted}
    \item[] {\makebox[2cm][l]{$P_{range}$} \% max. level the rightmost level of the subgraph can be}
   \item[]  {\makebox[2cm][l]{$N_{it,max}$} \%max.no.of iterations}
   %\item[]  {\makebox[2cm][l]{$\mathbf{u}$} \%tranmistted codeword}
   \item[]  {\makebox[2cm][l]{$stopI\!D$}  \%stopping criterion}
   \item[]  {\makebox[2cm][l]{$D$}  \%decoder specific parameters}
   \item[]  {\makebox[2cm][l]{$N_{min}$}}
   \end{itemize}
  }

  \Output
  {\begin{itemize}
  \setlength\itemsep{0em}
      \item [] {\makebox[2cm][l]{$\mathbf{\hat{u}}$} \%estimated codeword}
  \end{itemize}
  }

$N \longleftarrow  length(\mathbf{L}_{1,j})$\;
$n \longleftarrow \text{log}_2N$\;
$ (\mathbf{L},\mathbf{R}) \longleftarrow \mathbf{initializeLandR(\mathbf{L}_{1,j},\mathbb{A}})$\; 
$N_{it,reset} \longleftarrow \mathbf{initializeIterationResetValue}(N)$\;


\For{$iter\leftarrow 1$ \KwTo $N_{it,max}$}{
$ (\mathbf{L},\mathbf{R}) \leftarrow \mathbf{oneBPiteration(N, n, \mathbf{L}, \mathbf{R}},schedule)$\;


\If{$checkStopCondition(\mathbf{L},\mathbf{R},stopID)$}
{
$\mathbf{\hat{u}} = hardDecision(\mathbf{L}_{n+1,j}, \mathbf{R}_{n+1,j})$\;
$\mathbf{return \; \hat{u}}$
}
\If{$iter == N_{it,reset}$}
{
$\rho_{range} = randomRangeValue(P_{range})$\;
$\rho_{level} = randomLevelValue(P_{level}, \rho_{range})$\;
$schedule \leftarrow partialPermute(\rho_{range}, \rho_{level})$\;
$\mathbf{resetVariableNodes}(N,n,\mathbf{L}, \mathbf{R}, schedule)$\;
$N_{zero} = calcNumResetNodes(N, n, schedule)$\;
$N_{it,reset} = calcIterReset(N_{zero}, D, N_{min})$\;
$N_{it,reset} = iter+ N_{it, reset}$
}
}

$\mathbf{\hat{u}} = hardDecision(\mathbf{L}_{n+1,j}, \mathbf{R}_{n+1,j})$\;

 \caption{Partially Permuted Multi-Trellis BP decoding}
 \label{multitrellis}
\end{algorithm}


